Prototype Learning for Interpretable Respiratory Sound Analysis

Remote screening of respiratory diseases has been widely studied as a non-invasive and early instrument for diagnosis purposes, especially in the pandemic. The respiratory sound classification task has been realized with numerous deep neural network (DNN) models due to their superior performance. However, in the high-stake medical domain where decisions can have significant consequences, it is desirable to develop interpretable models; thus, providing understandable reasons for physicians and patients. To address the issue, we propose a prototype learning framework, that jointly generates exemplar samples for explanation and integrates these samples into a layer of DNNs. The experimental results indicate that our method outperforms the state-of-the-art approaches on the largest public respiratory sound database.

==> exp.tex <==
\section{Empirical Evaluation}

\input{exp_setup}

\input{exp_accuracy}


\input{exp_ablation}


\input{exp_sensitivity}

\input{exp_projection}

%\subsection{Qualitative Study}
%Any qualitative figures



%\subsection{Analysis of latent space}
%
%\sstitle{Setting}
%Show the quality of explanation, similar to section 2.6 of \cite{chen2019looks} and section V.B of \cite{chong2020towards}
%
%\sstitle{Results and discussion}


%\subsection{Reasoning process of our network}
%
%\sstitle{Setting}
%Similar to section 2.4 of \cite{chen2019looks}
%
%\sstitle{Results and discussion}



%\subsection{Some distinct experiment (Optional)}
%
%Some ideas: example ranking or example pruning (e.g. Figure 5(b) in \cite{chen2019looks})




==> exp_projection.tex <==
\subsection{Projection of Prototypes}
As the generated prototypes contain multiple channels and have a small spatial size due to local pooling layers, it is challenging to visualize the prototypes. Hence, we project the prototypes to their closest inputs of the models. Herein, the log Mel spectrograms calculated by the projection procedure for our best model on the test set are depicted in \autoref{fig:projection}. The projection of prototypes is helpful to analyse the characteristics of each class of respiratory sounds. We can see that, the \emph{normal} respiratory cycles are regular, while the others are not. The \emph{wheeze} log Mel spectrogram has smaller coefficients on a range of Mel frequncies than the \emph{crackle} one, probably indicating the \emph{wheeze} sound is weaker. 


\begin{figure}[ht]
%\vspace{-10pt}
\begin{subfigure}{.12\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/font_188_1b1_Ar_sc_Meditron_11_wav_y=0_dist_0.3167408.pdf}  
  \caption{Normal}
  \label{fig:sub-first}
\end{subfigure}
\hspace{-5pt}
\begin{subfigure}{.12\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/font_203_2p3_Pr_mc_AKGC417L_3_wav_y=1_dist_0.5895533.pdf}  
  \caption{Crackle}
  \label{fig:sub-second}
\end{subfigure}
\hspace{-5pt}
\begin{subfigure}{.12\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/font_158_1p3_Tc_mc_AKGC417L_0_wav_y=2_dist_0.4608453.pdf}  
  \caption{Wheeze}
  \label{fig:sub-second}
\end{subfigure}
\hspace{-5pt}
\begin{subfigure}{.12\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/font_180_1b4_Lr_mc_AKGC417L_0_wav_y=3_dist_1.3237557.pdf}  
  \caption{Both}
  \label{fig:sub-second}
\end{subfigure}
\vspace{-10pt}
\caption{The closest log Mel spectrograms to the prototypes. The X-axis is time frame and the Y-axis is Mel frequency.}
\label{fig:projection}
\vspace{-5pt}
\end{figure}



==> exp_setup.tex <==
\subsection{Experimental Settings}

\sstitle{Data}
The Scientific Challenge database released at the International Conference on Biomedical and Health Informatics (ICBHI) 2017~\cite{rocha2019open} is the largest publicly available collection of audio samples for respiratory sound classification. Totally $920$ audio recordings were collected from seven chest locations (\ie trachea, anterior left, anterior right, posterior left, posterior right, lateral left, and lateral right) of $126$ participants with four devices (\ie one microphone and three stethoscopes). The audio recordings have different sampling rates: $4$\, kHz, $10$\, kHz, and $44.1$\,kHz. All recordings derive $6\,898$ respiratory cycles, each of which was annotated with one of the four classes: \emph{normal}, \emph{crackle}, \emph{wheeze}, and \emph{both}, \ie \emph{crackle $+$ wheeze}. The database was split into a training set ($60\,\%$) and a test set ($40\,\%$) for the competition. 
To optimise the model hyperparameters, we further divide the training set into two subject-independent data sets: a train set ($70\,\%$) and a development set ($30\,\%$) (see \autoref{tab:datasets}). 


%\todo{Please fill here}

%\autoref{tab:datasets}

\begin{table}[!h]
    \centering
    \scriptsize
    \vspace{-5pt}
    \caption{Distribution of the splitted train/development sets and the official test set in the ICBHI database. }
    \label{tab:datasets}    
    \vspace{-10pt}
    \begin{tabular}{l|p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}}
    \toprule
         \#& \textbf{Normal} & \textbf{Crackle} & \textbf{Wheeze} & \textbf{Both} & $\bm{\sum}$ \\
         \hline
         \textbf{Train}& 1\,513 & \ \, 616 & 281 & 131 & 2\,541\\
         \textbf{Devel}& \ \, 550& \ \, 599 & 220 & 232 & 1\,601\\
         \textbf{Test} & 1\,579 & \ \, 649 & 385 & 143 & 2\,756 \\
         \hline
         $\bm{\sum}$ & 3\,642 & 1\,864 & 886 & 506 & 6\,898 \\
         \bottomrule
    \end{tabular}
    \vspace{-10pt}
\end{table}

\sstitle{Evaluation Metrics}
Although the database contains four labels, it is a common practice to differentiate abnormal cases (crackles, wheezes, and both) and normal cases. Therefore, the following standard benchmarks are used: \emph{sensitivity} (SE) -- equals to the number of true abnormal cases over the total number of abnormal cases, \emph{specificity} (SP) -- the ratio of true normal cases over normal cases, \emph{average score} (AS) -- is the official score of the ICBHI challenge~\cite{rocha2019open} and is the average of SE and SP. Due to class imbalance, we also report the \emph{unweighted average recall} (UAR) as the generic classification benchmark instead of \emph{accuracy}~\cite{song2021contrastive,ren2020generating}.

%\sstitle{Baselines} 
%To compare our proposed approach with the state-of-the-art (SOTA) methods on the ICBHI database, the implementation information of the SOTA methods are given as follows.
%\begin{compactitem}
%(1) \emph{MFCC-HG}~\cite{jakovljevic2017hidden}: The Mel-frequency cepstral coefficients (MFCCs) are extracted with their first derivatives as the input of the classifiers, which were structured with hidden Markov models (HMMs) and Gaussian mixture models (GMMs). 
%(2) \emph{MFCC-BDT}~\cite{chambres2018automatic}: The MFCCs from the audio signals are fed into a boosted decision tree (BDT) with four leaves for four classes.
%(3) \emph{STFT-WS}~\cite{serbes2017automated}: %Short-time Fourier transform (STFT) was applied to the channels produced by wavelet decomposition. 
%The frequency features integrated from the short-time Fourier transform (STFT) spectrograms and the statistical \& spectral features from the wavelet coefficients were classified by support vector machines (SVMs). 
%(4) \emph{STFT-WB}~\cite{ma2019lungbrn}: The STFT spectrograms and wavelet scalograms were extracted from the respiratory sounds and processed by a bi-ResNet model. 
%(5) \emph{STFT-RSESA}~\cite{yang2020adventitious}: The STFT spectrograms extracted from the audio signals were fed into a ResNet model with a squeeze-and-excitation (SE) block and a spatial attention (SA) block for the respiratory sound classification.
%\end{compactitem}


\sstitle{Implementation Details}
At the preprocessing stage, all audio recordings are resampled into $4$\,kHz due to the various sampling rates of the ICBHI database. A fifth butterworth bandpass filter ($100$\,Hz--$1\,800$\,Hz) is then applied to exclude noise components, \eg heart sounds, etc~\cite{rocha2019open}. The respiratory cycles with different durations are unified into audio signals with a fixed time length of $4$\,s. The log Mel spectrograms are further extracted from the audio signals with a window length of $256$, a hop length of $128$, and $128$ Mel bins, as they incorporate several properties of the human auditory system~\cite{martinez2014should}. %The static log Mel spectrograms, their deltas, and their delta-deltas are fed into the CNNs as the input. 

The CNN encoder is structured by four convolutional blocks with output channel numbers of $64$, $128$, $256$, and $512$, when each convolutional block consists of two covolutional layers with the same output channel number followed by a local max pooling layer with a kernel size of $2\times 2$. For classification, the CNN model with a CNN-encoder followed by a global max pooling layer and an FC layer is called `CNN-8'.

During training, the CNNs are optimised by an `Adam' optimiser with an initial learning rate of $0.001$ when the batch size is $16$. To stabilise the optmisation, the learning rate is reduced with a factor of $0.9$ at each $200$-th iteration. The training procedure is stopped at the $10\,000$-th iteration. To mitigate the class imbalance problem, each class in $\mathcal{L}_{NLL}$ is given a weight inversely proportional to the samples' number of the class. The value of $\alpha$ is experimentally set to $0.1$.


\sstitle{Reproducibility Environment}
Due to the page limitation, the technical report with more details of our work is available at: \url{https://arxiv.org/abs/2110.03536}. Our experiments are implemented at NVIDIA Geforce GTX 1080 Ti Graphics Cards. The PyTorch code is released at: \url{https://github.com/L3S/PrototypeSound}. 


==> method.tex <==
\section{Methodology}
\label{sec:method}
With the extracted log Mel spectrograms as well as their deltas and delta-deltas as the input, three prototype learning approaches are employed in our work: i) Prototype-1D, ii) Prototype-2D with vanilla similarity, and iii) Prototype-2D with attention-based similarity (see \autoref{fig:framework}). Before learning the prototypes in each approach, a CNN model is employed as an encoder for analysing the respiratory sounds due to CNNs' strong capability of extracting highly abstract representations. 
%The CNN encoder is followed by a global max pooling and a fully connected (FC) layer for the classification task when a prototype layer is not trained. 
%Next, the prototype layers in the three above approaches are described in detail.

\begin{figure}[!h]
    \centering
    \includegraphics[width=.95\linewidth]{figures/framework.pdf}
    \vspace{-10pt}
    \caption{The frameworks of the prototype learning. (a) Prototype-1D. (b) Prototype-2D with vanilla similarity. (c) Prototype-2D with attention-based similarity. BN = batch normalisation, FC = fully connected layer, LN = layer normalisation, RELU = rectified linear unit.}
    \label{fig:framework}
    \vspace{-20pt}
\end{figure}


\subsection{Prototype-1D}
As the high-level representations include more class-related information than the low-level ones, the prototype layer is trained after a global max pooling layer for 1D prototypes (see \autoref{fig:framework}(a)). Given an instance $(x, y)$ ($x$: input, $y$: label), the intermediate representation before the prototype layer is denoted by $f(x)$. Through the prototype layer, a set of prototypes $P_l, l\in [1;L]$ are learnt, where $L$ is the classes' number. In each $P_l$, $p_i,\ i\in[1;N]$ is a prototype with the same size of $f(x)$, where $N$ is the number of prototypes for each class. The cosine metric is then used to measure the similarities between $f(x)$ and $p_i$:
\begin{equation}
    S_{1D}(f(x),p_i)=\frac{f(x)^Tp_i}{\parallel f(x)\parallel_2\parallel p_i\parallel_2}.
\end{equation}
The similarity is further fed into a layer normalisation (LN) layer, a fully connected (FC) layer, and a softmax layer for classification. Although the prototype-1D can generate prototypes, it is challenging for 1D prototypes to represent the time and frequency information.

\subsection{Prototype-2D}
As 2D prototypes can better represent the time-frequency information than 1D prototypes, the prototype layer is placed after the CNN encoder for the similarity measurements (see \autoref{fig:framework}(b-c)).  

\sstitle{Vanilla Similarity}
Similar to the prototype-1D learning approach, the calculated similarities are send to the next layers for the classification task (see \autoref{fig:framework}(b)).

\sititle{Element-wise Similarity}
aims to calculate the similarity scores between each pair of time-frequency bins in $(f(x))$ and $p_i$. When $f(x)$'s channel number is $C$ and its spatial size is $(T, R)$, the element-wise similarity is calculated by
\begin{equation}
    S_{2EV}(f(x), p_i)=\sum_{c=1}^{C}\frac{f^{c,t,r}(x)p^{c,t,r}_i}{\parallel f^{c,t,r}(x)\parallel_2\parallel p^{c,t,r}_i\parallel_2},
\end{equation}
where $t\in[1;T]$ and ${r\in[1;R]}$.

\sititle{Average Similarity} is to compute an average score across the similarities between all time-frequency bins of $p_i$ and each bin of $f(x)$. Since only part of an audio signal may contain the class-related characteristics, the average similarity is a score between each $f(x)$ bin and $p_i$:
\begin{equation}
    S_{2AV}(f(x), p_i)=\mathop{\mbox{avg}}\limits_{t'=1,r'=1}^{T, R}\sum_{c=1}^{C}\frac{f^{c,t,r}(x)p^{c,t',r'}_i}{\parallel f^{c,t,r}(x)\parallel_2\parallel p^{c,t',r'}_i\parallel_2}.
\end{equation}


\sititle{Maximum Similarity}
has the same idea of the average similarity, but select the most similar $p_i$ bin for each $f(x)$ bin for structuring the similarity scores at all time-frequency bins. The maximum similarity is computed by
\begin{equation}
    S_{2MV}(f(x), p_i)=\max_{t'=1,r'=1}^{T, R}\sum_{c=1}^{C}\frac{f^{c,t,r}(x)p^{c,t',r'}_i}{\parallel f^{c,t,r}(x)\parallel_2\parallel p^{c,t',r'}_i\parallel_2}.
    \label{eq:2mv}
\end{equation}


\sstitle{Attention-based Similarity}
Apart from the vanilla similarity, the attention-based similarity (see \autoref{fig:framework}(c)) is employed to learn weighted similarity scores. The calculated similarity scores are processed by a softmax function $\sigma(\cdot)$ for the attention feature maps. As the average similarity is computed as a global score across all $p_i$ bins for each $f(x)$ bin, it is not applicable for the attention-based similarity. Therefore, we introduce the element-wise and maximum similarities with the attention mechanism.

\sititle{Element-wise Similarity}
is defined by
\begin{equation}
    S_{2EA}=\sum_{t=1,r=1}^{T, R}\sigma(S_{2EV}(f(x), p_i))f^{c,t,r}(x)p^{c,t,r}_i.
\end{equation}
%where $\sigma(\cdot)$ is the softmax function.

\sititle{Maximum Similarity} is calculated at each $(f(x))$ bin $f^{c,t,r}(x)$ and its most similar $p_i$ bin $p^{c,t_{max},r_{max}}_i$ in Equation~(\ref{eq:2mv})
\begin{equation}
    S_{2MA}=\sum_{t=1,r=1}^{T, R}\sigma(S_{2MV}(f(x), p_i))f^{c,t,r}(x)p^{c,t_{max},r_{max}}_i.
\end{equation}


\subsection{Training}
During training the above prototype learning models, the prototypes are learnt as part of the model parameters. The loss function of the neural networks is finally defined by
\begin{equation}
    \mathcal{L}=\mathcal{L}_{NLL}+\alpha\mathcal{L}_{dv},
\end{equation}
\begin{equation}
    \mathcal{L}_{dv}= \frac{\mathop{\mbox{avg}}_{l_1=1,l_2=1}^{L,L} S_{2AV}(P_{l_1}, P_{l_2})}{\mathop{\mbox{avg}}_{l=1}^{L} S_{2AV}(P_l, P_l)}, l_1\neq l_2,
\end{equation}
where $\mathcal{L}_{NLL}$ is the negative log likelihood (NLL) loss function when the neural networks' output in \autoref{fig:framework} is passed into a logarithm function, $\mathcal{L}_{dv}$ denotes the diverse loss function, and $\alpha$ is a constant value. $\mathcal{L}_{dv}$ aims to reduce the distances among prototypes which represent the same class and increase the distances among prototypes for different classes. 



==> related.tex <==
\section{Related Work}
\label{sec:related}


\sstitle{Respiratory Sound Classification}
\cite{song2021contrastive}


\sstitle{Example-based Explanation}
\edit{One of the earliest works in  learning by example is the k-nearest neighbor (k-NN) classifier~\cite{coluccia2020robust}. In the recent years, researchers have proposed to combine DNNs with example-based classifiers. Another work~\cite{chen2019looks} introduced a prototypical part network (ProtoPNet) that is able to present the prototypical cases that are similar to the parts the network looks at. These explanations are used during classification and not created posthoc.~\cite{chong2020towards}}

Mostly limited to image domain.
